MNELLS: The MUSE Nearby Early-Type Galaxy Lens Locator Survey

Low-redshift strong-lensing galaxies can provide robust measurements of the stellar mass-to-light ratios in early-type galaxies (ETG), and hence constrain variations in the stellar initial mass function (IMF). At present, only a few such systems are known. Here, we report the first results from a blind search for gravitationally-lensed emission line sources behind 52 massive $z$ $<$ 0.07 ETGs with MUSE integral field spectroscopy. For 16 galaxies, new observations were acquired, whilst the other 36 were analysed from archival data. This project has previously yielded one confirmed galaxy-scale strong lens (J0403-0239) which we report in an earlier paper. J0403-0239 has since received follow-up observations, presented here, which indicate support for our earlier IMF results. Three cluster-scale, and hence dark-matter-dominated, lensing systems were also discovered (central galaxies of A4059, A2052 and AS555). For nine further galaxies, we detect a singly-imaged but closely-projected source within 6 arcsec (including one candidate with sources at three different redshifts); such cases can be exploited to derive upper limits on the IMF mass-excess factor, $\alpha$. Combining the new lens and new upper limits, with the previously-discovered systems, we infer an average $\langle \alpha \rangle$ = 1.06 $\pm$ 0.08 (marginalised over the intrinsic scatter), which is inconsistent with a Salpeter-like IMF ($\alpha$ = 1.55) at the 6$\sigma$ level. We test the detection threshold in these short-exposure MUSE observations with the injection and recovery of simulated sources, and predict that one in twenty-five observations is expected to yield a new strong-lens system. Our observational results are consistent with this expected yield.

==> storage.tex <==
\section{Discussion}
\label{sec:Disc}



\subsection{Modifications to the target selection}
\label{sec:TS_alt}

The results presented in this paper can be used as a tool to improve the target selection







\subsection{Lensing Analysis - More than expected?}
\label{sec:LAmte}


In this Section we will compare the results from this paper to our predictions, and to the MaNGA survey \citep{Bundy2015}. For any calculation, a typical massive ETG lens has a lensing cross section of 23\,arcsec$^{2}$.

%In this Section we will compare our predictions for the lens search to the results which have been presented here. We will also compare our search technique to the MaNGA survey. It is targeting a large number of ETGs, with a median redshift of $\langle z \rangle$\,=\,0.05, and therefore will serendipitously discover a number of gravitational strong lenses comparable to the SNELLS and MNELLS sample. Our aim for the MNELLS sample was to discover three new low-$z$ lenses, and in this Section we discuss this compared to our results. For our calculations, a typical massive ETG lens has a lensing cross section of 23\,arcsec$^{2}$.

The initial predictions for our detection threshold took flux limits from the MUSE exposure time calculator (ETC), and applied them to the MUSE-wide survey numbers. We predicted 23.5 emitters per arcmin$^{2}$, which converts to 0.15 lensed emitters per target. This value was not reached, due to our poor-weather programme negatively impacting the expected seeing. Applying our measured detection threshold revised the prediction to 15.4 emitters per arcmin$^{2}$ from the MUSE-wide observations. This revised estimate results in 0.10 lensed emitters per target. Using our observations, the results from 14 full depth cubes is 12.66 emitters per arcmin$^{2}$ leaving 0.08 lensed emitters per target. Finally, when we include the detection threshold limit within the central 5\,arcsec, reduces the number density to 9.3 emitters per arcmin$^{2}$, and 0.06 lensed emitters per target. This is almost half of the prediction using MUSE-wide and our overall flux limit, but for the full 26 galaxies would still predict 1.6\,$\pm$\,1 new strong-lenses (uncertainty from binomial statistics). 

Although this new predicted number of lenses is lower than expected, there are a few contributions which need to be considered in a future targeted survey. We appear to detect less emitters than we would expect from the MUSE-wide number counts, even with the actual measured detection limit. This potentially suggests that our chosen targets lay in regions of low background large-scale structure, or the fields within the MUSE-wide survey are more densely populated. However, the standard deviation of 5.5 from our data, suggests that there is extremely large scatter in the number counts within a 1\,arcminute$^{2}$ MUSE pointing. With only 14 full depth cubes, the large scatter still suggests that it is possible that we will match our predictions from the MUSE-wide after our full survey is complete. Finally, the centre of our cubes are dominated by massive foreground elliptical galaxies, which are significantly less present in the MUSE-wide fields. Hence, this may also impact the effective area on the sky which we probe to a comparable detection threshold, something that was not taken into account for our initial predictions.

Although the central flux threshold is higher, `Upper limit lensing' increases the area around each galaxy which can contain an emitter and be valuable for investigating the IMF. We did not take this into account for our initial predictions, and the new area incorporates twice R$_{\rm Ein}$. The new area is four times larger, totalling 92\,arcsec$^{2}$, including the area in which a single source can be detected without a counter image (Some of this area also includes the double-imaged regime). Therefore incorporating this new area with our number counts, we expect that one in three MNELLS targets will be single-imaged but closely projected or double-imaged systems.

The full MaNGA survey will target over 10\,000 ETGs with a median redshift of $\langle\,z\,\rangle$\,=\,0.05, using an IFU, and therefore will serendipitously discover a number of low-$z$ gravitational strong lenses. \citet{Talbot2018} work with a sample of 2812 ETGs, and so far has produced only a handful of candidate lenses. A key difference is the ETGs which are being targeted. Where our selection criteria lead us to observe the most massive field ETGs in the local universe, MaNGA target a broad spectrum of galaxy sizes, and hence contain many low-$\sigma$ ETGs which relatively have much smaller strong-lensing volumes. In addition, the MaNGA selection favours larger, (higher-$\sigma$), ETGs which lie at higher redshift, so that they cover the same \reff\ \citep[See Fig.8,][]{Bundy2015}. This has two main implications, firstly low-$\sigma$ galaxies are less likely to be lenses, and their impact on the understanding of the IMF is much lower (The discrepancy between SLACS and SNELLS is at high-$\sigma$, low-$\sigma$ appear to have little scatter). Secondly a higher redshift lens is more likely to have an R$_{\rm Ein}$ which is a significant fraction of it's R$_{\rm Eff}$, which complicates the disentangling of the DM component. 


If the MaNGA survey discovers a statistically significant sample of ETG strong lenses, a large proportion will not be comparable to the high-$\sigma$ SLACS, SNELLS or MNELLS lenses, and therefore will have less impact on our understanding the IMF discrepancy. Furthermore the resolution of the MaNGA data may require additional follow-up observations (see Smith et al. in prep). 



To date ManGA has only discovered 2-4 lenses in 2812 observed galaxies, which scaled to the full six-year sample (10,000 galaxies) will be approximately 10. A direct comparison to SNELLS and MNELLS plus the archival search, which totals of order 100 observations, we have discovered four confirmed low-$z$, high-$\sigma$ strong-lenses (With an additional three cluster-scale lenses). Therefore it appears the targeted survey is currently the most efficient technique for yielding a statistically significant population of these lenses.


%it appears that the total number of lenses within the full six-year sample (10,000 galaxies) will be approximately 10. Comparing this to SNELLS, MNELLS and an archival search which have discovered 4 lenses in just over 100 observations (With an additional three cluster-scale lenses), it appears that this technique will yield far more lenses with far fewer hours of observations. 




%The MaNGA survey has been used to attempt to discover new low-$z$ lenses. \citet{Talbot2018} work with a sample of 2812 ETGs, and they discover less than 5 lenses. A key difference is the ETGs being targeted. We target the most massive field ETGs in the local universe, which have the largest lensing cross-section and hence a higher likelihood of being a lens. Where as MaNGA target a broad spectrum of galaxy sizes, and hence contain many low-$\sigma$ ETGs which have much smaller lensing background volume. In addition, due to the selection based on $i$-band absolute magnitude, the high-$\sigma$ ETGs tend to lie at higher redshift. Furthermore, when specifically considering the case for investigating the IMF, these galaxies are less informative, as there appears to be very little scatter at low-$\sigma$, and hence discovering new high-$\sigma$ lenses are key to understanding why there appears to be variation with $\sigma$. Hence, although the MaNGA survey has high scientific output in a range of fields, specifically for finding low-$z$ massive ETG strong lenses, it is inefficient due to the higher contribution at low-$z$ from low-likelihood lens galaxies. 



%With ManGA having only discovered 2-4 lenses in 2812 observed galaxies, it appears that the total number of lenses within the full six-year sample (10,000 galaxies) will be approximately 10. Comparing this to SNELLS, MNELLS and an archival search which have discovered 4 lenses in just over 100 observations (With an additional three cluster-scale lenses), it appears that this technique will yield far more lenses with far fewer hours of observations. 

